Super homologies associated with low dimensional Lie algebras

A Poisson structure on a manifold is characterized by the Schouten bracket. The graded algebra of the tangent bundle with the Schouten bracket is a prototype of Lie superalgebra. The Poisson condition means that a cycle in the 2-chain space. Given a graded Lie superalgebra, the 0-graded subspace is a Lie algebra. In this note, using the DGA of tangent bundle with the Schouten bracket as a model, we start from an abstract Lie algebra, construct non-trivial Lie superalgebra by Schouten-like bracket. Then it is natural to ask how the core Lie algebra control the Lie superalgebra. One trial here is to investigate the Betti numbers of the super homology groups. For abelian Lie algebras, the boundary operator is trivial, so we study super homology groups for low dimensional non-abelian Lie algebras of dimension smaller than 4.

==> G3D3-A1-src.tex <==
\section{$ \dim[\frakg,\frakg]=3$ and $A_{1}$-type}


\renewcommand{\arraystretch}{1.0}
\setlength{\arraycolsep}{4pt}

We fix the 2-vector basis \( \ub{1} = \frac{1}{2} \zb{1} \wedge \zb{3}\), 
 \( \ub{2} = \frac{-1}{2} \zb{2} \wedge \zb{3}\), 
 \( \ub{3} =  \zb{1} \wedge \zb{2}\), and 3-vector 
by \( \zb{4} = V= \zb{1} \wedge \zb{2} \wedge \zb{3} \).   
The 
multiplication (by the Schouten bracket) tables are the followings: 
\begin{center}
\( \begin{array}[t]{c|*{3}{c}|c|*{3}{c} }
 & \zb{1} & \zb{2} & \zb{3} & \zb{4}& \ub{1} & \ub{2} & \ub{3}  
 \\\hline 
\zb{1} & 0 & \zb{3}  & 2 \zb{1} & 0  & 0 & \ub{3} & 2\ub{1}   \\
\zb{2} & -\zb{3}  & 0 & - 2\zb{2}& 0  &  - \ub{3} & 0 & -2 \ub{2} \\
\zb{3} & - 2\zb{1} & 2 \zb{2} & 0 & 0  &  -2 \ub{1} & 2\ub{2}  & 0
\end{array}
 \)
\hfil
\( \begin{array}[t]{c|*{3}{c}|c}
   & \ub{1} & \ub{2} & \ub{3} & \zb{4} 
\\\hline 
\ub{1} & 0 &  - \zb{4} & 0 & 0 \\
\ub{2} & - \zb{4} & 0 & 0 & 0 \\
\ub{3} & 0 & 0  &  2\zb{4}  & 0\\
\end{array}
 \)
\end{center}

%\end{document} \endinput 

Then we have 
\begin{align*}
\pdel W^{1111} &= 0\;,\quad 
\pdel W^{1110} = 0 \;,\quad 
\\
\pdel W^{1101} &= \zb{3} \mywedge \zb{4} \;,\quad 
\pdel W^{1011} =  2 \zb{1} \mywedge \zb{4}\;,\quad 
\pdel W^{0111} =  -2 \zb{2} \mywedge \zb{4}\;,\quad 
\\
%
\pdel U^{a,b,c} &= \zb{4} \mywedge (
-  a b  U^{a-1, b-1, c}
+  2 \binom{c}{2}  U^{a, b, c-2} )
\;. 
\\
\sum_{A} \LC{i}{A}\pdel U^{a,b,c} &= \zb{4} \mywedge \sum_{} U^{p,q,r} (
-(p+1)(q+1) \LC{i}{p+1, q+1, r} 
+  (r+2)(r+1)    \LC{i}{p, q, r+2} )
\;. 
\\
\SbtES{\zb{1}}{U^{A}} &=  b U^{a,b-1,c+1} + 2c U^{a+1,b,c-1}\;,\quad  
\\
\sum_{A} \LC{i}{A} \SbtES{\zb{1}}{U^{A}} 
&= \sum_{A}((b+1)\LC{i} {a,b+1,c-1} + 2 (c+1)\LC{i}{a-1,b,c+1}) U^{A}\;,
\\
\SbtES{\zb{2}}{U^{A}} &= - a U^{a-1,b,c+1} - 2c U^{a,b+1,c-1} \\
\sum_{A} \LC{i}{A} \SbtES{\zb{2}}{U^{A}} 
&= \sum_{A}(- (a+1)\LC{i} {a+1,b,c-1} - 2 (c+1)\LC{i}{a,b-1,c+1}) U^{A}\;,
\\
\SbtES{\zb{3}}{U^{A}} &= 2(-a +  b)U^{a,b,c} 
\end{align*}


\paragraph{The kernel space of \(\wtedC{w+3}{w}\):} 
%We study the kernel space of \(\wtedC{w+3}{w}\).
Take a general chain 
\(L =  \sum_{a+b+c=w} \LC{}{a,b,c} W^{1,1,1,0} \mywedge U^{a,b,c}\) with
unknown scalars \(\LC{}{a,b,c} \). 
%\(\ds W^{1100} \mywedge \sum  \LC{}{A}  \SbtES{\zb{3}}{U^{A}}\)
\begin{align*} 
\pdel L =&  \pdel ( \sum_{A} \LC{}{A}  W^{1110} \mywedge U^{A})
\\=& \sum \LC{}{a,b,c} ( \pdel   W^{1,1,1,0})  \mywedge U^{A}
-  W^{1110} \mywedge \sum \LC{}{A}  \pdel U^{A}
+ \sum_{i=1}^{3} (-1)^{i+1} W^{ \eps{i}=\eps{4}=0 } \sum \LC{ }{A}\SbtES{ \zb{i} } { U^{A
} }
\\ 
=& 
- W^{1111} \mywedge \sum  (  -  (p+1)(q+1) \LC{}{p+1,q+1,r} 
+  (r+2)(r+1)  \LC{}{p,q,r+2} )U^{p, q, r}
\\& 
 + \zb{2} \mywedge \zb{3} \mywedge \sum  ( 
(b+1)\LC{}{a,b+1,c-1} + 2 (c+1) \LC{}{a-1,b,c+1}
) U^{a,b,c}
\\& 
- \zb{1} \mywedge \zb{3} \mywedge \sum ( 
- (a+1) \LC{}{a+1,b,c-1} - 2 (c+1)\LC{}{a,b-1,c+1} 
)U^{a,b,c}
+ \zb{1} \mywedge \zb{2} \mywedge \sum \LC{ }{A} 2( -a + b  )  U^{a,b,c}
\end{align*} 
The linear equation 
\( \pdel L =0\) is generated by the followings:  
\begin{subequations}
\begin{align}
& (p+1)(q+1)\LC{}{p+1,q+1,r } - (r+2)(r+1) \LC{}{p,q,r+2 } \label{G3:D3:t2:a}
\\
 & 
(b+1) \LC{ }{a,b+1,c-1}  + 2 (c+1) \LC{ }{a-1,b,c+1}  \label{G3:D3:t2:b}
\\& 
 (a+1) \LC{ }{a+1,b,c-1} + 2 (c+1) \LC{ }{a,b-1,c+1}  \label{G3:D3:t2:c}
\\& 
2( -a + b ) \LC{ }{a,b,c}  \label{G3:D3:t2:d}
\end{align} 
\end{subequations}

When \(w=0\), then the unknown parameter is only one \(\LC{}{0,0,0}\)
and the above equations give no information. This means  \(\LC{}{0,0,0}\)
is free, and so the kernel dimension is 1.  In fact, \( \pdel ( \zb{1}
\mywedge \zb{2}
\mywedge \zb{3}) =0 \). 

When \(w=1\), the unknown parameters  are \(\LC{}{a,b,c}\)
with \(a+b+c=1\). \eqref{G3:D3:t2:a} gives no information, but  
\eqref{G3:D3:t2:d} tells 
\( \LC{}{1,0,0} =0\) , \( \LC{}{0,1,0} =0\).   
\( \LC{}{0,0,1} =0\) comes from 
\eqref{G3:D3:t2:b} by \((a,b,c)=(1,0,0)\). 
Thus, the kernel dimension is 0.  

Now assume \(w \geqq 2\). From \eqref{G3:D3:t2:d}, we see that 
\( \LC{}{a,b,c} = 0 \)  if  \( b \ne c \). 
We gather 
\eqref{G3:D3:t2:a} $\sim$
\eqref{G3:D3:t2:c} with  the first and  second arguments
are equal. 
\begin{subequations}
\begin{align}
& (p+1)^ 2\LC{}{p+1,p+1,r } - (r+2)(r+1) \LC{}{p,p,r+2 } \label{G3:D3:t2:Aa}
\\
 & 
(b+1) \LC{ }{b+1,b+1,c-1}  + 2 (c+1) \LC{ }{b,b,c+1}  \label{G3:D3:t2:Ab}
\\& 
 (a+1) \LC{ }{a+1,a+1,c-1} + 2 (c+1) \LC{ }{a,a,c+1}  \label{G3:D3:t2:Ac}
\end{align}
\end{subequations}
 \eqref{G3:D3:t2:Ab}
 and 
 \eqref{G3:D3:t2:Ac} are the same equations. 
 \eqref{G3:D3:t2:Aa}
 and 
 \eqref{G3:D3:t2:Ab}, we conclude \(  \LC{}{a+1,a+1,c-1} = 0\)
and  \(  \LC{}{a,a,c-1} = 0\). Thus, the kernel dimension is 0. 


\bigskip


\paragraph{The kernel space of \(\wtedC{w+2}{w}\):} 
We study the kernel space of \(\wtedC{w+2}{w}\). 
\kmcomment{where  
the generators are  \( W[\eps{i}=\eps{4}=0]
\mywedge \bU{a,b,c}{w}\)
or \( W^{1,1,1,1} \mywedge \bU{p,q,r}{w-2}\).   
}
Take a general chain \(L+M\) with 
\(L= \sum \LC{i}{a,b,c}  W[{\eps{i}=\eps{4}=0}] \mywedge \bU{a,b,c}{w}
\) and \( M= 
 \sum \MC{} {p,q,r}  W^{1111} \mywedge \bU{p,q,r}{w-2}
\) with unknown scalars \(\LC{i}{a,b,c}, \MC{}{p,q,r}\).   
Then 
\begin{align*}
& \pdel (L+ M) \\
= & 
 \sum \LC{i}{A}( \pdel( W[{\eps{i}=\eps{4}=0}]) \mywedge U^{A}
+  W[{\eps{i}=\eps{4}=0}] \mywedge  \pdel U^{A} )
+ \SbtES{
W[{\eps{i}=\eps{4}=0}] } { U^{A} } 
 \\& 
+ 0 + 0 + \sum \MC{} {P}  \SbtES{ W^{1111}}{ U^{P}}  
\\ 
\kmcomment{  
=&    
- 2 \zb{2} \mywedge\sum \LC{1}{A} U^{A}
+ 2 \zb{1} \mywedge\sum \LC{2}{A} U^{A}
+  \zb{3} \mywedge\sum \LC{3}{A} U^{A}
\\& 
+ W^{0111}\mywedge\sum\LC{1}{A}(-ab U^{a-1,b-1,c}+2\binom{c}{2}U^{a,b,c-2}) 
\\& 
+ W^{1011}\mywedge\sum\LC{2}{A}(-ab U^{a-1,b-1,c}+2\binom{c}{2}U^{a,b,c-2}) 
\\& 
+ W^{1101}\mywedge\sum\LC{3}{A}(-ab U^{a-1,b-1,c}+2\binom{c}{2}U^{a,b,c-2}) 
\\& 
+ \sum \LC{1}{A} ( - \zb{2} \SbtES{ \zb{3} }{ U^{A} }
                   + \zb{3} \SbtES{ \zb{2} }{ U^{A} } )
+ \sum \LC{2}{A} ( - \zb{1} \SbtES{ \zb{3} }{ U^{A} }
                   + \zb{3} \SbtES{ \zb{1} }{ U^{A} } )
                   \\& 
+ \sum \LC{3}{A} ( - \zb{1} \SbtES{ \zb{2} }{ U^{A} }
                   + \zb{2} \SbtES{ \zb{1} }{ U^{A} } )
\\&
+ W^{0111} \mywedge \MC{}{P} \SbtES{ \zb{1} }{ U^{P} } 
- W^{1011} \mywedge \MC{}{P} \SbtES{ \zb{2} }{ U^{P} } 
+ W^{1101} \mywedge \MC{}{P} \SbtES{ \zb{3} }{ U^{P} } 
\\
} 
= & 
+  \zb{1} \mywedge\sum ( 2 \LC{2}{A} U^{A}
 -  \LC{2}{A} \SbtES{ \zb{3} }{ U^{A} }
 -  \LC{3}{A} \SbtES{ \zb{2} }{ U^{A} }
 )
\\& 
+  \zb{2} \mywedge\sum (- 2 \LC{1}{A} U^{A}
  -  \LC{1}{A}\SbtES{ \zb{3} }{ U^{A} }
 +  \LC{3}{A} \SbtES{ \zb{1} }{ U^{A} } 
 )
\\& 
+  \zb{3} \mywedge\sum ( \LC{3}{A} U^{A}
  +  \LC{1}{A}\SbtES{ \zb{2} }{ U^{A} } 
 +  \LC{2}{A} \SbtES{ \zb{1} }{ U^{A} } 
 )
%%%%%%%%%%%%%%%%%%%
\\& 
+ W^{0111} \mywedge \sum ( \MC{}{P} \SbtES{\zb{1}}{U^{P}} 
- \LC{1}{A} ab  U^{a-1,b-1,c}+2\tbinom{c}{2}\LC{1}{A} U^{a,b,c-2})  
\\& 
+ W^{1011} \mywedge \sum (- \MC{}{P} \SbtES{\zb{2}}{U^{P}} 
- \LC{2}{A} ab  U^{a-1,b-1,c}+2\tbinom{c}{2} \LC{2}{A} U^{a,b,c-2}) 
\\& 
+ W^{1101} \mywedge\sum ( \MC{}{P} \SbtES{\zb{3}}{U^{P}} 
- \LC{3}{A} ab U^{a-1,b-1,c}+2\tbinom{c}{2}\LC{3}{A} U^{a,b,c-2})  
\\
= & 
+  \zb{1} \mywedge\sum U^{A}( 
 2(1+a+b)   \LC{2}{A}  
 + (a+1) \LC{3}{a+1,b,c-1}  +2(c+1) \LC{3}{a,b-1,c+1})
 )
\\& 
+ \zb{2} \mywedge\sum  U^{A} (
    \LC{1}{A} (-2 +2a-2b) 
 + (b+1) \LC{3}{a,b+1,c-1}  + 2 (c+1) \LC{3}{a-1,b,c+1} )
 )
\\& 
+  \zb{3} \mywedge\sum U^{A} ( \LC{3}{A} 
  - (a+1) \LC{1}{a+1,b,c-1} -2(c+1)  \LC{1}{a,b-1,c+1} 
 +  (b+1)\LC{2}{a,b+1,c-1} + 2 (c+1) \LC{2}{a-1,b,c+1}  )
%%%%%%%%%%%%%%%%%%%
\\& 
+ W^{0111} \mywedge \sum U^{P}( 
        ( q+1) \MC{}{p,q+1,r-1}  + 2 (r+1) \MC{}{p-1,q,r+1}  
- \LC{1}{p+1,q+1,r} (p+1)(q+1)  +2\tbinom{r+2}{2}\LC{1}{p,q,r+2} )  
\\& 
+ W^{1011} \mywedge \sum U^{P} ( 
 (p+1) \MC{}{p+1,q,r-1}  +2(r+1) \MC{}{p,q-1,r+1}
- \LC{2}{p+1,q+1,r} (p+1)(q+1)  +2\tbinom{r+2}{2}\LC{2}{p,q,r+2} )  
) 
\\& 
+ W^{1101} \mywedge\sum U^{P} ( \MC{}{P} (-2p+2q) 
- \LC{3}{p+1,q+1,r} (p+1)(q+1)  +2\tbinom{r+2}{2}\LC{3}{p,q,r+2} )  
)  
\end{align*}
%
Then \( \pdel (L+M) =0\) is defined by the following polynomials of unknown
\(\LC{i}{A}\) and \(\MC{}{P}\): 
\begin{subequations}
\begin{align}
E_{1} =&   2(1+a-b)   \LC{2}{a,b,c}  
 + (a+1) \LC{3}{a+1,b,c-1}  +2(c+1) \LC{3}{a,b-1,c+1} 
\label{G3:D3:type2:CwP2:a}
\\
E_{2} = & 
  2(-1 + a - b) \LC{1}{a,b,c} 
 + (b+1) \LC{3}{a,b+1,c-1}  + 2 (c+1) \LC{3}{a-1,b,c+1} 
\label{G3:D3:type2:CwP2:b}
\\
E_{3} = & 
 \LC{3}{a,b,c} 
  - (a+1) \LC{1}{a+1,b,c-1} -2(c+1)  \LC{1}{a,b-1,c+1} 
 +  (b+1)\LC{2}{a,b+1,c-1} 
\label{G3:D3:type2:CwP2:c} \\& + 2 (c+1) \LC{2}{a-1,b,c+1}  \notag
%%%%%%%%%%%%%%%%%%%
\\
E_{4} = & 
        ( q+1) \MC{}{p,q+1,r-1}  + 2 (r+1) \MC{}{p-1,q,r+1}  
- \LC{1}{p+1,q+1,r} (p+1)(q+1) 
\label{G3:D3:type2:CwP2:d} \\&  + (r+2)(r+1) \LC{1}{p,q,r+2} \notag  
\\
E_{5} = & 
(p+1) \MC{}{p+1,q,r-1}  +2(r+1) \MC{}{p,q-1,r+1}
- \LC{2}{p+1,q+1,r} (p+1)(q+1) 
\label{G3:D3:type2:CwP2:e} \\& + (r+2)(r+1) \LC{2}{p,q,r+2}   \notag
\\
E_{6} = & 
  \MC{}{P} (-2p+2q) 
- \LC{3}{p+1,q+1,r} (p+1)(q+1) + (r+2)(r+1) \LC{3}{p,q,r+2}   
\label{G3:D3:type2:CwP2:f}
\end{align}
\end{subequations}

\eqref{G3:D3:type2:CwP2:c} tells that \( \LC{3}{A}\) are completely
determined by \( \LC{1}{A}, \LC{2}{A}\). 
From \eqref{G3:D3:type2:CwP2:f},  we have linearly independent generators
with leading term \( \MC{}{p,q,r}\) with \( p\ne q\), which cardinality is
\( \binom{w}{2} - \# \{ (p,p,r) \mid 2 p+r=w-2  \}\).  
Since 
\begin{align*} E_{4}(p,p-1,r) =& p \MC{}{p,p,r-1} + 2(r+1) \MC{}{p-1,p-1,r+1}
\\& - p(p+1) \LC{1}{p+1,p, r}
+ (r+2)(r+1) \LC{1}{p,p-1, r+2}\\\shortintertext{and} 
E_{5}(p-1,p,r) =& p \MC{}{p,p,r-1} + 2(r+1) \MC{}{p-1,p-1,r+1} \\& 
 - p(p+1) \LC{2}{p,p+1, r}
+ (r+2)(r+1) \LC{2}{p-1,p, r+2}\end{align*}  
we keep generators with leading term \(
\MC{}{p,p,r}\), we got \(\tbinom{w}{2}\) linearly independent generators with leading term
\(\MC{}{p,q,r}\). 
We have to check 
\( \widehat{E}_{1} =  E_{1} \mod  E_{3} \), 
\( \widehat{E}_{2} =  E_{2} \mod  E_{3} \), 
and \( \widehat{E}_{6} =  E_{6} \text{ with } p=q \mod E_{3} \). 
%
\begin{align} 
\widehat{E}_{1} = & (a+2) (a+1) \LC{1}{a+2,b,c-2} + 4 (c+2) (c+1) \LC{1}{a,
b-2,c+2} +2 (2 c+1) (a+1) \LC{1}{a+1,b-1,c}  \label{HE:1}\\&
-(b+1) (a+1) \LC{2}{a+1,b+1,c-2} - 4 (c+2) (c+1) \LC{2}{a-1,b-1,c+2}\notag \\& 
+ 2 (- a c- b c + a -2b - c+1)\LC{2}{a,b,c} \notag \\ 
%
\widehat{E}_{2} =&  (b+1) (a+1)  \LC{1}{a+1,b+1,c-2} +4 (c+2) (c+1)  \LC{1}
{a-1,b-1,c+2}  \label{HE:2} \\&
+ 2 ( a c + b c+2 a- b+ c-1) \LC{1}{a,b,c}
-(b+2) (b+1)  \LC{2}{a,b+2,c-2}\notag\\&
-4 (c+2) (c+ 1)  \LC{2}{a-2,b,c+2}
-2 (2 c+1) (b+1) \LC{2}{a-1,b+1,c} \notag\\ 
%
\widehat{E}_{6} =& -(a+2) (a+1)^2  \LC{1}{a+2,a+1,c-1} -(c+1) (a+1) (2 a-c)
\LC{1} {a+1, a, c+1} \label{HE:3}\\& 
+ 2 (c+3) (c+2) (c+1) \LC{1}{a,a-1,c+3} + (a+2) (a+1)^2  \LC{2}
{a+1,a+2, c-1} 
\notag\\& 
+ (c +1) (a+1) (2 a-c)  \LC{2}{a,a+1,c+1} -2 (c+3) (c+2)
(c+1) \LC{2}{a-1,a,c+3} \notag
\end{align}
%
We take the subspace \( S \) generated by \( \LC{1}{a,b,c} - 
\LC{2}{a-1,b+1,c}\) inspired from \eqref{HE:3}. Then 
\begin{align*}
\widehat{E}_{6}\hspace{-5pt} \mod
S &= 0\\  
 \widehat{E}_{1} \hspace{-5pt} \mod S &= (a-b+1) ( (a+1) \LC{2} {a+1,b+1,c-2} + 2(c+2)
 \LC{2}{a,b,c})  \\
\widehat{E}_{2} \hspace{-5pt} \mod S &= (a-b-1) ( (b+1) \LC{2} {a,b+2,c-2} + 2(c+2)
 \LC{2}{a-1,b+1,c}) \end{align*}
 
Thus, we claim the dimension of the space generated by \(\widehat{E}_{1},
\widehat{E}_{2}, \widehat{E}_{3} \)   is \( 2\tbinom{w+2}{2}\), and the
total rank is   \( \tbinom{w}{2}+ 2\tbinom{w+2}{2}\). 

\kmcomment{
% old, original basis

We pick up the coefficient of \(W^{\varE} \mywedge U^{a,b,c}\):   
\begin{subequations}
\begin{align}
 W^{1,0,0,0} & : \quad  \LC{2}{a,b,c}(  (1+\alpha)a + b+ \alpha c + 1
) - \alpha \LC{3}{a-1,b+1,c} (b+1)   \label{f:0:a}
\\ 
 W^{0,1,0,0} & : \quad  \LC{1}{a,b,c}(
 (1+\alpha)a + b+ \alpha c  + \alpha  )
 - \LC{3}{a-1,b,c+1} (c+1)  \label{f:0:b}
\\ 
 W^{0,0,1,0}& : \quad   \alpha  \LC{1}{a-1,b+1,c}  (b+1) 
- \LC{2}{a-1,b,c+1} (c+1)  \label{f:0:c}
\\ 
 W^{0,1,1,1} & : \quad -  \MC{ }{p-1,q,r+1} (r+1) 
 + (1-\alpha) \LC{1}{p,q+1,r+1} (q+1) (r+1) 
 \label{f:0:d}
\\ 
 W^{1,0,1,1} & : \quad  
 - \alpha  \MC{ }{p-1,q+1,r} (q+1) 
 + (1-\alpha) \LC{2}{p,q+1,r+1} (q+1) (r+1) 
\label{f:0:e}
\\ 
 W^{1,1,0,1}& :  \quad  
- \MC{ }{p,q,r}( (1+\alpha)(p+2) + q+ \alpha r  )
 + (1-\alpha) \LC{3}{p,q+1,r+1} (q+1) (r+1) 
 \label{f:0:f}
\end{align}
\end{subequations}

Assume \(\alpha=1\).  Then  
\eqref{nf:0:d} and 
\eqref{nf:0:e} imply  \( \MC{}{p,q,r} =0 \) if \( q + r > 0\). 
We put \((p,q,r)= (w-2,0,0)\) to \eqref{nf:0:f}, then 
 \( \MC{}{w-2,0,0}2w  =0 \). Thus,  \( \MC{}{p,q,r} =0 \) when \(
 w > 0\).  

\eqref{nf:0:a} and 
\eqref{nf:0:b} imply \[
\LC{2}{a,b,c} = \frac{\alpha (a+1)}{w+c+1} \LC{3}{a+1,b,c-1} \;,\;
\LC{1}{a,b,c} = \frac{ b+1}{w+c+1} \LC{3}{a,b+1,c-1} \;,\;\]
and \eqref{nf:0:c} holds. Thus, the free variables of 
\( \MC{}{p,q,r}, \LC{i}{a,b,c} \) are 
\( \LC{3}{a,b,c} \), and the freedom (the kernel dimension) is
\(\binom{w+2}{2}\). 

Now assume \( \alpha \ne 1\). 
Then \eqref{f:0:d},  \eqref{f:0:e} and \eqref{f:0:f} yield 
\( \LC{i}{a,b,c} \)  with \( b c > 0\)  are expressed by \(\MC{}{p,q,r}\).  
Before dealing with the cases of \( bc=0\), we show visible relations
from \eqref{f:0:a},  \eqref{f:0:b} and \eqref{f:0:c}.  
\begin{center}
\begin{tikzpicture}[scale=0.35]
\node at (0,4) {slant relation}; 
\draw[lightgray] (0,0) grid (1,1); 
\draw 
node at (0,1) {$\blacksquare$} 
node [above left] at (0,1) {$\LC{3}{a,b,c}$} 
node  at (1,0) {$\bullet$} 
node [below right] at (1,0) {$\LC{2}{a+1,b-1,c}$}; 
\end{tikzpicture}
\hfil
\begin{tikzpicture}[scale=0.35]
\node at (0,4) {horizontal relation}; 
\draw[lightgray] (0,0) grid (1,0); 
\draw 
node at (0,0) {$\blacksquare$} 
node [above left] at (0,0) {$\LC{3}{a,b,c}$} 
node  at (1,0) {$\diamondsuit$} 
node [below right] at (1,0) {$\LC{1}{a+1,b,c-1}$}; 
\end{tikzpicture}
\hfil
\begin{tikzpicture}[scale=0.35]
\node at (0,4) {vertical relation}; 
\draw[lightgray] (0,0) grid (0,1); 
\draw 
node at (0,1) {$\diamondsuit$} 
node [above left] at (0,1) {$\LC{1}{a,b,c}$} 
node  at (0,0) {$\bullet$} 
node [below right] at (0,0) {$\LC{2}{a,b-1,c+1}$}; 
\end{tikzpicture}
\end{center} 

About \(\LC{1}{a,0,c}\): By horizontal relation, 
\(\LC{1}{a,0,c}\) with $a>0$ is expressed by 
\(\LC{3}{a-1,0,c+1}\). Putting \(a=b=0\) for \eqref{f:0:b}, we have 
\( \LC{1} {0,0,w} \alpha (w+1) =0\), i.e., 
\( \LC{1} {0,0,w}  =0\). Thus, 
there is no freedom for \(\LC{1}{a,0,c}\). 

About \(\LC{2}{a,b,0}\): By slant relation, 
\(\LC{2}{a,b,0}\) with $a>0$ is expressed by 
\(\LC{3}{a-1,b+1,0}\). Putting \(a=c=0\) for \eqref{f:0:a}, we have 
\( \LC{2} {0,w,0}  (w+1) =0\), i.e., 
\( \LC{2} {0,w,0}  =0\). Thus, 
there is no freedom for \(\LC{2}{a,b,0}\). 


\begin{wrapfigure}[5]{r}[0.5cm]{0.4\textwidth}
\vspace{-\baselineskip}
%\centering
\begin{tikzpicture}[scale=0.4]
\foreach \y in {0,-1,...,-6} \draw[lightgray] (0, \y) -- ( - \y,\y ) -- ( - \y,-6 ); 
\draw[lightgray] ( 0,0 ) -- ( 6, -6 ) 
      ( 0,-1 ) -- ( 6-1, -6 )
;

\foreach \y in {0,-1,...,-4} \node[] at   ( - \y,\y )  {$\diamondsuit$}; 
\foreach \y in {0,-1,...,-4} \node[] at   ( - \y,\y -1 )  {$\bullet$} ; 

\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.4]
\foreach \y in {0,-1,...,-6} \draw[lightgray] (0, \y) -- ( - \y,\y ) -- ( - \y,-6 ); 
\draw[lightgray] ( 0,0 ) -- ( 6, -6 ) 
      ( 0,-1 ) -- ( 6-1, -6 )
;

\foreach \y in {-1,-2,...,-5} \node[] at   ( - \y,\y )  {$\diamondsuit$}; 
\foreach \y in {-1,-2,...,-5} \node[] at   ( -1 - \y,\y  ) {$\blacksquare$} ; 

\end{tikzpicture}
\end{wrapfigure}
\strut 
About \(\LC{1}{a,b,0}\): The left-side picture says \(\LC{1}{a,b,0} \)
($b>1$) is expressed by \(\LC{2}{a,b-1,1}\) and so expressed by \(\MC{}
{p,q,r}\). From the right picture, we check the horizontal relation
\eqref{f:0:b} when \(b=1, c=0\). Then we get 
\( \LC{1}{w-1,1,0}(1+\alpha) w - \LC{3}{w-2,1,1} = 0\).  
If \( 1+ \alpha \ne 0\), 
\( \LC{1}{w-1,1,0} = \frac{1}{(1+\alpha) w } \LC{3}{w-2,1,1} \)  and
expressed by \( \MC{}{p,q,r}\). 
If \( 1+ \alpha = 0\), there is no relation about 
\( \LC{1}{w-1,1,0}\) (and  \(\LC{3}{w-2,1,1} = 0 \)). 
Thus, the freedom of 
\( \LC{1}{a,b,c}\) with \(bc=0\) is  1 if \(\alpha +1 =0\) given by
\(\LC{1}{w-1,1,0}\), otherwise 0.  


\begin{wrapfigure}[5]{r}[0.5cm]{0.4\textwidth}
\vspace{-\baselineskip}
%\centering
\begin{tikzpicture}[scale=0.4]
\foreach \y in {0,-1,...,-6} \draw[lightgray] (0, \y) -- ( - \y,\y ) -- ( - \y,-6 ); 
\draw[lightgray] ( 0,0 ) -- ( 6, -6 ) %( 0,-1 ) -- ( 6-1, -6 ) 
;

\foreach \y in {0,-1,...,-4} \node[] at   ( - \y, -5 )  {$\diamondsuit$}; 
\foreach \y in {0,-1,...,-4} \node[] at   ( - \y, -6 )  {$\bullet$} ; 

\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.4]
\foreach \y in {0,-1,...,-6} \draw[lightgray] (0, \y) -- ( - \y,\y ) -- ( - \y,-6 ); 
\draw[lightgray] ( 0,0 ) -- ( 6, -6 ) % ( 0,-1 ) -- ( 6-1, -6 )
;

\foreach \y in {-1,-2,...,-5} \node[] at   ( - \y, -6 )  {$\bullet$}; 
\foreach \y in {-1,-2,...,-5} \node[] at   ( -1 - \y,-5  ) {$\blacksquare$} ; 

\end{tikzpicture}
\end{wrapfigure}
\strut
About \(\LC{2}{a,0,c}\): By the almost same argument, 
 the freedom of 
\( \LC{2}{a,b,c}\) with \(bc=0\) is  1 if \(\alpha +1 =0\) given by
\(\LC{2}{w-1,0,1}\), otherwise 0.  
\(\LC{2}{w-1,0,1}\) is expressed by 
\(\LC{1}{w-1,1,0}\) through vertical relation, and vice versa. Thus, the
total generators of 
\( \MC{}{p,q,r}, \LC{i}{a,b,c} \) are 
\( \MC{}{p,q,r}\) and \(\LC{3}{a,b,c} \) with \( bc = 0\) and \(\kappa\)
, which appeared in Remark \ref{remark:parameter} and the freedom
(kernel dimension) is   
\( \binom{w}{2} + 2(w+1) -1 + \kappa = \binom{w+2}{2} + \kappa\). 
}%endOFkmcomment
%



\paragraph{The kernel space of \(\wtedC{w+1}{w}\):} 
When \(w=0\), then \(\wtedC{w+1}{w} = \wtedC{1}{0} = \frakg\) and the
boundary operator is trivial, and so the kernel dimension is \(\dim
\frakg\). We then 
study the kernel space for \(w > 0\).  
Take a general chain \(L+M\) where \( L = \sum \LC{i}{a,b,c}  \zb{i}
\mywedge \bU{a,b,c}{w}\) and \( M = \sum \MC{i} {p,q,r} W[\eps{i}=0 ]
\mywedge \bU{p,q,r}{w-2} \) with unknown scalars \(\LC{i}{a,b,c}, \MC{i}{p,q,
r}\).   
\begin{align*}
\pdel(L+M) =& \sum \LC{i}{A} (
- \zb{i}\mywedge \pdel\bU{A}{w} + \SbtES{\zb{i}}{\bU{A}{w}}) 
+ \sum \MC{j}{P} (( \pdel W[\eps{j}=0] ) \mywedge \bU{P}{w-2} 
+ \SbtES{ W[\eps{j}=0] }{\bU{P}{w-2}} )
\\
\kmcomment{  
=& - \sum \zb{i} \mywedge \zb{4} \mywedge U^{p,q,r} (   
 - (p+1) (q+1) \LC{i}{p+1,q+1,r} + 2 \tbinom{r+2}{2} \LC{i}{p,q,r+2})
+\sum \LC{i}{A} \SbtES{ \zb{i} } {U^{A}}
\\& 
+ \zb{2} \mywedge \zb{4}\mywedge \sum (-2) \MC{1}{P} U^{P}
+ \zb{1} \mywedge \zb{4}\mywedge\sum 2 \MC{2}{P} U^{P}
+ \zb{3} \mywedge \zb{4}\mywedge\sum  \MC{3}{P} U^{P}
\\& 
+ \sum \MC{1}{P} ( 
  \zb{3} \mywedge \zb{4} \mywedge \SbtES{ \zb{2} } {U^{P}}
- \zb{2} \mywedge \zb{4} \mywedge \SbtES{ \zb{3} } {U^{P}}
)
\\& 
+ \sum \MC{2}{P} ( 
  \zb{3} \mywedge \zb{4} \mywedge \SbtES{ \zb{1} } {U^{P}}
- \zb{1} \mywedge \zb{4} \mywedge \SbtES{ \zb{3} } {U^{P}}
)
\\& 
+ \sum \MC{3}{P} ( 
  \zb{2} \mywedge \zb{4} \mywedge \SbtES{ \zb{1} } {U^{P}}
- \zb{1} \mywedge \zb{4} \mywedge \SbtES{ \zb{2} } {U^{P}}
) 
\\ %aa
} 
=&  
+\sum \LC{i}{A} \SbtES{ \zb{i} } {U^{A}}
\\& 
+ \zb{1} \mywedge \zb{4} \mywedge\sum ( U^{p,q,r} (   
  (p+1) (q+1) \LC{1}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{1}{p,q,r+2})
+  2 \MC{2}{P} U^{P}
\\& 
- \MC{2}{P} \SbtES{ \zb{3} } {U^{P}}
- \MC{3}{P} \SbtES{ \zb{2} } {U^{P}}
)
\\& 
+ \zb{2} \mywedge \zb{4} \mywedge ( U^{p,q,r} (   
  (p+1) (q+1) \LC{2}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{2}{p,q,r+2})
+ (-2) \MC{1}{P} U^{P}
\\& 
- \MC{1}{P} \SbtES{ \zb{3} } {U^{P}}
+ \MC{3}{P} \SbtES{ \zb{1} } {U^{P}}
)
\\& 
+ \zb{3} \mywedge \zb{4} \mywedge ( U^{p,q,r} (   
  (p+1) (q+1) \LC{3}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{3}{p,q,r+2})
+  \MC{3}{P} U^{P}
\\& 
+  \MC{1}{P} \SbtES{ \zb{2} } {U^{P}}
+  \MC{2}{P} \SbtES{ \zb{1} } {U^{P}}
)
\\ %bb
=&  
%+\sum \LC{i}{A} \SbtES{ \zb{i} } {U^{A}}
+\sum U^{A} (  (b+1) \LC{1}{a,b+1,c-1} + 2(c+1) \LC{1}{a-1,b,c+1}  
-(a+1) \LC{2}{a+1,b,c-1} - 2(c+1) \LC{2}{a,b-1,c+1}  
\\& \quad 
+ (-2a + 2 b) \LC{3}{a,b,c} 
)
\\& 
+ \zb{1} \mywedge \zb{4} \mywedge\sum  U^{p,q,r} (   
  (p+1) (q+1) \LC{1}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{1}{p,q,r+2})
+  2 \MC{2}{P} 
\\& \quad 
- \MC{2}{P} (-2p+2q) 
-  (-(p+1)\MC{3}{p+1,q,r-1}-2(r+1)\MC{3}{p,q-1,r+1})
)
\\& 
+ \zb{2} \mywedge \zb{4} \mywedge  U^{p,q,r} ( (  
  (p+1) (q+1) \LC{2}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{2}{p,q,r+2})
+ (-2) \MC{1}{P} 
\\& \quad 
- \MC{1}{P} ( -2p+2q )
+  ((q+1)\MC{3}{p,q+1,r-1} +2(r+1)\MC{3}{p-1,q,r+1})
)
\\& 
+ \zb{3} \mywedge \zb{4} \mywedge  U^{p,q,r} (   
  (p+1) (q+1) \LC{3}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{3}{p,q,r+2}
+  \MC{3}{P} 
\\& \quad 
+   (-(p+1)\MC{1}{p+1,q,r-1}-2(r+1)\MC{1}{p,q-1,r+1})
+   ((q+1)\MC{2}{p,q+1,r-1} +2(r+1)\MC{2}{p-1,q,r+1})
)
\end{align*} %NHK1
Thus, the linear equation \( \pdel (L+M) =0\) is defined by 
%
\begin{subequations}
\begin{align}
G_{0} =&  (b+1) \LC{1}{a,b+1,c-1} + 2(c+1) \LC{1}{a-1,b,c+1}  
-(a+1) \LC{2}{a+1,b,c-1} - 2(c+1) \LC{2}{a,b-1,c+1}  
\label{G3:D3:type2:w+1:0}
\\& \qquad 
+ (-2a + 2 b) \LC{3}{a,b,c} 
\notag
\\
%
G_{1} =& 
(p+1) (q+1) \LC{1}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{1}{p,q,r+2}
\label{G3:D3:type2:w+1:1}
\\& \qquad 
+  (2+2p-2q) \MC{2}{P} 
+(p+1)\MC{3}{p+1,q,r-1}+2(r+1)\MC{3}{p,q-1,r+1}
\notag \\
%
G_{2} =& 
  (p+1) (q+1) \LC{2}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{2}{p,q,r+2}
\label{G3:D3:type2:w+1:2}
\\& \qquad 
+ (-2+2p-2q) \MC{1}{P} 
+  (q+1)\MC{3}{p,q+1,r-1} +2(r+1)\MC{3}{p-1,q,r+1}
\notag
\\
% 
G_{3} = &
(p+1) (q+1) \LC{3}{p+1,q+1,r} - 2 \tbinom{r+2}{2} \LC{3}{p,q,r+2}
+  \MC{3}{p,q,r} 
   -(p+1)\MC{1}{p+1,q,r-1}
\label{G3:D3:type2:w+1:3}
\\& \qquad -2(r+1)\MC{1}{p,q-1,r+1}
+   (q+1)\MC{2}{p,q+1,r-1} +2(r+1)\MC{2}{p-1,q,r+1}  
\notag
\end{align} %NHK2
\end{subequations}
If we focus on  \(\MC{3}{p,q,r}\) in \eqref{G3:D3:type2:w+1:3} and
substitute it into  \eqref{G3:D3:type2:w+1:1} and \eqref{G3:D3:type2:w+1:2},  
then we have next equations without \( \MC{i}{P}\):
\begin{align}
H_{1} = &     (b+1) (a+1)  \LC{1}{a+1,b+1,c} -(c+2) (c+1) \LC{1}{a,b,c+2}
-(a+2)  (a+1) (b+1) \LC{3}{a+2,b+1,c-1} \label{G3:D3:type2:w+1:H1} 
\\& 
-(c+1) (-c+2 b) (a+1)  \LC{3}{a+1,b,c+1}
+2 (c+3)  (c+2) (c+1) \LC{3}{a,b-1,c+3}
\notag
\\
H_{2} =&     (b+1) (a+1)  \LC{2}{a+1,b+1,c}-(c+2) (c+1)  \LC{2}{a,b,c+2}
-(b+2)  (b+1) (a+1)  \LC{3}{a+1,b+2,c-1} \label{G3:D3:type2:w+1:H2} 
\\& 
-(c+1) (b+1) (2 a-c)  \LC{3}{a,b+1,
c+1} + 2 (c+3)  (c+2) (c+1)  \LC{3}{a-1,b,c+3}\notag  
\end{align}
Now we look for the dimension of the space generated by \( G_{0}\), \( H_{1}
\) and \( H_{0}\).  If \( a \ne b \), then \(\LC{3}{a,b,c}\) is determined
by \(\LC{1}{A}\) and \(\LC{2}{A}\) by \eqref{G3:D3:type2:w+1:0}. 
About  \(\LC{3}{a,a,c}\),  they are also determined
by \(\LC{1}{A}\) and \(\LC{2}{A}\) by \eqref{G3:D3:type2:w+1:H1} and  
\eqref{G3:D3:type2:w+1:H2}. Thus, the kernel dimension is \( \binom{w}{2} + 2
\binom{w+2}{2}\).  

\kmcomment{

Oo := (p,q,r) -> 
- (
(p+1)* (q+1)* N[p+1,q+1,r] - (r+2)*(r+1)*   N[p,q,r+2]
 # + O[p,q,r] 
   -(p+1)* P[p+1,q,r-1]-2*(r+1)*P[p,q-1,r+1]
+   (q+1)* Q[p,q+1,r-1] +2*(r+1)*Q[p-1,q,r+1] )  ; 



(* 
hh1 := {[(b+1)*(a+1), L[a+1,b+1,c]], [-(c+2)*(c+1), L[a,b,c+2]]}, {}, {[-(a+2)
*(a+1)*(b+1), N[a+2,b+1,c-1]], [-(c+1)*(-c+2*b)*(a+1), N[a+1,b,c+1]], [2*(c+3)
*(c+2)*(c+1), N[a,b-1,c+3]]}, {}, {};

hh2 := {}, {[(b+1)*(a+1), M[a+1,b+1,c]], [-(c+2)*(c+1), M[a,b,c+2]]}, {[-(b+2)
*(b+1)*(a+1), N[a+1,b+2,c-1]], [-(c+1)*(b+1)*(2*a-c), N[a,b+1,c+1]], [2*(c+3)*
(c+2)*(c+1), N[a-1,b,c+3]]}, {}, {};
*) 

H1 := (a,b,c) ->  (b+1)*(a+1)* L[a+1,b+1,c] -(c+2)*(c+1) * L[a,b,c+2]
-(a+2) *(a+1)*(b+1)*N[a+2,b+1,c-1]-(c+1)*(-c+2*b)*(a+1)* N[a+1,b,c+1]
+2*(c+3) *(c+2)*(c+1)*N[a,b-1,c+3]:

H2 := (a,b,c) ->  
(b+1)*(a+1)* M[a+1,b+1,c]-(c+2)*(c+1)* M[a,b,c+2]
-(b+2) *(b+1)*(a+1)* N[a+1,b+2,c-1]-(c+1)*(b+1)*(2*a-c)* N[a,b+1,c+1] +
2*(c+3)* (c+2)*(c+1)* N[a-1,b,c+3] : 


HH1 := (a,b,c) ->  (b+1)*(a+1)* L[a+1,b+1,c] -(c+2)*(c+1) * L[a,b,c+2]
-(a+2) *(a+1)*(b+1)*NN(a+2,b+1,c-1)-(c+1)*(-c+2*b)*(a+1)* NN(a+1,b,c+1)
+2*(c+3) *(c+2)*(c+1)*NN(a,b-1,c+3):

HH2 := (a,b,c) ->  
(b+1)*(a+1)* M[a+1,b+1,c]-(c+2)*(c+1)* M[a,b,c+2]
-(b+2) *(b+1)*(a+1)* NN(a+1,b+2,c-1)-(c+1)*(b+1)*(2*a-c)* NN(a,b+1,c+1) +
2*(c+3)* (c+2)*(c+1)* NN(a-1,b,c+3) : 

}



\paragraph{The kernel space of \(\wtedC{w}{w}\):} 
When \(w=0\), then \(\wtedC{w}{w} = \Lambda ^{0}\frakg\) and the
boundary operator is trivial, and so the kernel dimension is 1.  
We study the kernel space of \(\wtedC{w}{w}\)  for \(w > 0\).  
Take a general chain \(L+M\) where \( L = \sum \LC{ }{A}
\bU{A}{w}\) and \( M = \sum \MC{i} {P}  \zb{i} \mywedge \zb{4}
\mywedge \bU{P}{w-2} \) with unknown scalars \(\LC{ }{A},
\MC{i}{P}\).   
\begin{align*}
\pdel(L+M) =&  \sum \LC{}{A} \pdel U^{A} 
+ 0 + 0 
+ \sum \MC{j}{P} \zb{4} \mywedge \SbtES{\zb{j}}{U^{P}}
\\
=&  \zb{4} \mywedge\sum U^{p,q,r} (
-(p+1)(q+1)\LC{}{p+1,q+1,r}
+ 2 \tbinom{r+2}{2} \LC{}{p,q,r+2}
\\&\qquad 
+ (q+1) \MC{1}{p,q+1,r-1} + 2(r+1) \MC{1}{p-1,q,r+1}
- (p+1) \MC{2}{p+1,q,r-1} - 2(r+1) \MC{2}{p,q-1,r+1}
\\&\qquad 
+ ( -2p+2q ) \MC{3}{p,q,r}
)
\end{align*}
Thus, the linear equations \( \pdel(L+M)=0\) is defined by 
\begin{align}
& \label{HHK:A1:0:a}
-(p+1)(q+1)\LC{}{p+1,q+1,r}
+ 2 \tbinom{r+2}{2} \LC{}{p,q,r+2}
\\&\qquad 
+ (q+1) \MC{1}{p,q+1,r-1} + 2(r+1) \MC{1}{p-1,q,r+1}
- (p+1) \MC{2}{p+1,q,r-1} - 2(r+1) \MC{2}{p,q-1,r+1}
\notag \\&\qquad 
+ ( -2p+2q ) \MC{3}{p,q,r}
\notag
\end{align}
\kmcomment{ \textcolor{red}{Revised} on July 21, 2020 by focusing the rank,
the number of generators of linear equations: }
The space is decomposed into direct product of two subspaces, one is defined
by \(p\ne q\) and the other is defined by \(p=q\). 
The space defined by \(p \ne q\) has a basis with leading term \( \MC{3}{p,
q,r} \) and so the dimension is \( \binom{w}{2} - \# \{ (p,p,r) \mid
2p+r=w-2 \}\).  The other space is generated by 
\begin{align*} 
& -(p+1)(p+1)\LC{}{p+1,p+1,r}
+ 2 \tbinom{r+2}{2} \LC{}{p,p,r+2}
\\&\qquad 
+ (p+1) \MC{1}{p,p+1,r-1} + 2(r+1) \MC{1}{p-1,p,r+1}
- (p+1) \MC{2}{p+1,p,r-1} - 2(r+1) \MC{2}{p,p-1,r+1}
\end{align*} 
and we see the dimension is 
 \( \# \{ (p,p,r) \mid 2p+r = w-2\}\). Thus, 
the rank is \( \binom{w}{2}\), and the kernel dimension is \( 2\binom{w}{2}
+ \binom{w+2}{2}\).  






\paragraph{The kernel space of \(\wtedC{w-1}{w}\):} 
Generators of this chain space are \( \zb{4}\mywedge \bU{A}{w-2}\). 

Since 
\(\pdel (\zb{4}\mywedge \bU{A}{w-2}) = 
- \zb{4}\mywedge \pdel(\bU{A}{w-2}) + \SbtES{\zb{4}}{ \bU{A}{w-2}} 
= - \zb{4} \mywedge \zb{4} \wedge  (1-\alpha ) b c \bU{a,b-1,c-1}{w-2} 
+ 0 = 0 \), the boundary operator is trivial and the kernel dimension is 
\( \binom{w}{2}\). 


\renewcommand{\arraystretch}{1.3}


\paragraph{Final table of chain complex }
\begin{center}
\(
\begin{array}{c|*{5}{c}}
\text{weight}= w > 0 & w-1 & w & w+1 & w+2 & w+3\\\hline
\text{SpaceDim} & 
\binom{w}{2} & 
3 \binom{w}{2} + \binom{w+2}{2} & 
3\binom{w}{2} + 3\binom{w+2}{2} & 
\binom{w}{2} + 3\binom{w+2}{2} & 
\binom{w+2}{2} 
\\
\ker\dim & \binom{w}{2} & 2\binom{w}{2}  +\binom{w+2}{2}  & 
\binom{w}{2} + 2 \binom{w+2}{2}   & \binom{w+2}{2}  & 0   \\\hline
\text{Betti} & 0 & 0 &  0  & 0   &  0 
\end{array}
\)
\end{center}
\endinput

%\end{document} 


